Radial Dependence of Extinction in Parent Galaxies of Supernovae

The problem of extinction is the most important issue to be dealt with in the process of obtaining true absolute magnitudes of core-collapse (including stripped-envelope) supernovae (SNe). The plane-parallel model, widely used in the past, was shown not to describe extinction adequately. We try to apply an alternative model which introduces radial dependance of extinction in parent galaxies of supernovae. For calculating extinction in our Galaxy we use two different methods and compare the results obtained. Our analysis is primarily focused on a chosen sample of stripped-envelope SNe (Ib/c) for which we find intrinsic peak absolute magnitude $\mathrm{M}_{\mathrm{B}}^{0}=-17.80\pm 0.43$.

==> readme <==
-------------------------
THE REVMEXAA LATEX MACROS
-------------------------

Version: 3.17 (08 Apr 2003)

Author: William Henney (w.henney@astrosmo.unam.mx)

Latest version available from:	http://www.astrosmo.unam.mx/rmaa


USAGE
-----

All you need to use this package is the file `rmaa.cls' 

On the other hand, you may find the User Guide and sample documents
instructive.  If you get errors while compiling the example files,
please look in the OLDLATEX/ directory for up-to-date versions of
various required packages.


DOCUMENTATION
-------------

Please note that the User Guide has not been updated since
version 2.x of the macros.  The example document rm-ex1.tex has some
more up-to-date instructions. A few more last-minute hints are given
in the release notes below. 


VERSION 3.1x RELEASE NOTES 
--------------------------

Versions 3.1x require a relatively recent LaTeX installation.  If your
LaTeX is more than a few years old you may get some errors when
compiling the example documents. To help such cases, I have provided
up-to-date versions of some of the required style files in the
directory OLDLATEX/. Copy any that you need to somewhere LaTeX can
find them (e.g., your working directory). If you still have problems,
please contact me (w.henney@astrosmo.unam.mx).

You can now use natbib to do your citations. An example will be coming
soon. In the meantime, you can read natbib's documentation (try typing
`texdoc natbib' - it might work) or follow the same instructions as
for the aastex macros. Note that aastex ships with a very old version
of natbib.sty - if necessary you may need to grab the more recent
version from the OLDLATEX/ directory.

The file rmaacite.sty is no longer included in the distribution for
authors (it is still included in the distribution for editors). You
shouldn't use this package for new articles (use natbib instead - it
is much better). To compile old documents that do use rmaacite.sty, you
must now add the `nonatbib' option to the \documentclass command.

If you have appendices to your article, you can use 

\begin{appendices}

\section{First Appendix}
\label{sec:ap-A}

Blah, blah, blah. 

\section{Second Appendix}
\label{sec:ap-B}

Etcetera.

\end{appendices}

This goes after the acknowledgements but before the
bibliography. Equations in appendices will be labelled A1, A2, B1, B2,
etc. 

FILE MANIFEST for rmaaN.MM.tar:
-------------------------------

README			this file
rmaa.cls		LaTeX class file for typesetting RMAA articles 
rmuser.tex		Guide for Authors (very out of date)
rm-ex1.tex		Example proceedings paper and tutorial
rm-ex2.tex		Example poster paper
example-fig.eps		Example of postscript figure
example-badfig.eps	Example of how not to do a postscript figure
GPL			Terms and conditions for copying, distribution
                        and modification
OLDLATEX/		Directory containing some style files that will
			let you use the macros even if you have an 
			not-quite-cutting-edge version of LaTeX
	


